Situated and Interactive Multimodal Conversations

Next generation virtual assistants are envisioned to handle multimodal inputs (e.g., vision, memories of previous interactions, in addition to the user's utterances), and perform multimodal actions (e.g., displaying a route in addition to generating the system's utterance). We introduce Situated Interactive MultiModal Conversations (SIMMC) as a new direction aimed at training agents that take multimodal actions grounded in a co-evolving multimodal input context in addition to the dialog history. We provide two SIMMC datasets totalling ~13K human-human dialogs (~169K utterances) using a multimodal Wizard-of-Oz (WoZ) setup, on two shopping domains: (a) furniture (grounded in a shared virtual environment) and, (b) fashion (grounded in an evolving set of images). We also provide logs of the items appearing in each scene, and contextual NLU and coreference annotations, using a novel and unified framework of SIMMC conversational acts for both user and assistant utterances. Finally, we present several tasks within SIMMC as objective evaluation protocols, such as Structural API Prediction and Response Generation. We benchmark a collection of existing models on these SIMMC tasks as strong baselines, and demonstrate rich multimodal conversational interactions. Our data, annotations, code, and models are publicly available.

==> tex_modules/archive.tex <==

\textbf{Multi-Modal Dialog State Tracking (MM-DST)}: We extend the traditional notion of the unimodal dialog state tracking (DST) problem and propose a new task where slots are grounded on the coexisting multi-modal context, which requires handling of multi-modal objects (as opposed to textual tokens) as part of dialog states. Consider as a motivating example the following dialog  initiated with the user utterance “Does \underline{this} come in blue?”, accompanied with the visual scene with a black dress as a focused item. The traditional DST tracks the item of the conversational focus (“\underline{this}”) as a textual token, which fails to capture its canonical reference (the actual object in view) as a slot that is often required for subsequent API queries to be successful, \eg “Is \underline{it} more expensive than the other blue dress I saw from H\&M?” Therefore, in the proposed MM-DST, we require that each model produces a reference pointer to the object, in addition to textual spans or tokens. Given user utterances, we will evaluate the model’s performance on intent prediction, slot prediction, and coreference resolution.

\textbf{Multi-Modal Dialog Evaluation}: We invite the community to help build evaluation methods/metrics specifically for multi-modal conversational AI systems. We will provide the fine-grained ground-truth annotations and human evaluation for diverse aspects of each dialog as a reference. We propose evaluating these automated methods of validating component level as well as overall end-to-end dialog generation and action prediction by estimating their correlations to human annotations. This task is motivated by the recent interest in building automated evaluation techniques such as \cite{Lowe+17, Daudaravicius+16}. Similar tasks have been pursued in domains such as machine translation.




\section{Tasks}
\label{subsec:tracks}

\todo{Change the wording as potential tasks that people could work on with this dataset; probably shouldn't mention MM-DST too much though to avoid overlap with the future follow-up paper (e.g. EMNLP submission)}


\begin{table*}[t]
    \begin{center}
        \scalebox{0.9}{
        \setlength\tabcolsep{9pt}
        \begin{tabular}{p{0.28\textwidth}p{0.35\textwidth}p{0.25\textwidth}}
        \toprule[\heavyrulewidth]
        \textbf{Task Name}  & \textbf{Description} & \textbf{Evaluation} \\
        \midrule
        1. Multi-modal Dialog State Tracking & See below & Intent Accuracy,
Slot Precision / Recall / F1, Coref Precision / Recall / F1 \\
        \midrule
        2. Assistant action selection (Structural API call prediction) & Given user utterances, we evaluate the models’ performance on retrieving correct API(s). & Perplexity, Mean Average Precision, (Human Evaluation) \\
        \midrule
        3. Response Generation & Given user utterances and/or ground-truth APIs, we evaluate the performance on the assistant response generation (generation and retrieval). & Generation: BLEU, Perplexity, Human Evaluation (Naturalness, etc.); Retrieval: Accuracy@k, Entropy \\
        \midrule
        4. User Satisfaction Prediction & We evaluate the performance on the user satisfaction score prediction task at a dialog level. & Accuracy, Macro/Micro-F1, Precision, Recall \\
        \midrule
        5. Multi-modal Dialog Evaluation & See below & Correlation to human evaluation \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \vspace{-6pt} 
    \caption{\textbf{Proposed tracks and descriptions}}
    \vspace{-10pt}   
    \label{tab:tracks}
\end{table*}




==> tex_modules/tables/api_call_list_doublecolumn.tex <==
\begin{table*}[t]
    \begin{center}
        \scalebox{0.8}{
        \setlength\tabcolsep{5pt}
        \begin{tabular}{
            p{0.18\textwidth}p{0.40\textwidth}p{0.40\textwidth}
        }
        \toprule[\heavyrulewidth]
        \textbf{API Name}  & \textbf{Furniture} & \textbf{Fashion} \\
        \midrule
        Search Item & 
        \textit{SearchFurniture}: Search furniture items in the database using category, 
        color, intended room, material, and price range (min--max) attributes.
        &
        \textit{SearchDatabase}: Search in the database of images for the current task.
        \linebreak
        \textit{SearchMemory}: Search in the user memory images.
        \\
        \midrule
        Get Information &
        \textit{GetInfo}: Get additional information about an 
        \\
        \midrule
        \textit{Domain-specific APIs}
        & 
        N/A 
        & 
        \textit{FocusOnFurniture}:
        \linebreak
        \textit{RotateFurniture}:
        \linebreak
        \textit{NavigateCarousel}: Move the carousel back and forth to navigate through 
        the search results.  \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    %\vspace*{\captionReduceTop}
    \caption{
        List of APIs supported in our \simmc dataset for both furniture and fashion domains.
    }
    \vspace*{\captionReduceBot}
    \label{tab:api_call_list}
\end{table*}

==> tex_modules/tables/model_components_all.tex <==
%p{0.18\textwidth}p{0.40\textwidth}p{0.40\textwidth}
\begin{table}[t]
    \begin{center}
        \scalebox{0.9}{
        \setlength\tabcolsep{5pt}
        \begin{tabular}{p{0.09\textwidth} p{0.1\textwidth} p{0.1\textwidth} p{0.1\textwidth} p{0.1\textwidth}}
        \toprule[\heavyrulewidth]
        \textbf{Model}
        & \textbf{Utterance/History \newline Encoder}
        & \textbf{Multimodal \newline Fusion} 
        & \textbf{Action \newline Predictor} 
        & \textbf{Response \newline Generator}\\
        \midrule
        History-Agnostic (HAE)
        &$
            \displaystyle
            \begin{aligned}
                u_t &= \text{LSTM}(U_t) \\
                h_t &= \phi
            \end{aligned}
        $ 
        & \multirow{3}{*}{
            $
            \displaystyle
            \begin{aligned}
                m_t &= \text{Attn}(M_t, u_t) \\
                \tilde{u}_t &= [m_t; u_t]
            \end{aligned}
        $
        }
        &
        $
            \displaystyle
            \begin{aligned}
                q_t &= \text{MLP}(\tilde{u}_t) \\
                p_t &= \text{Softmax}(q_t) \\
                \hat{a}_t &= \text{argmax}(p_t)
            \end{aligned}
        $ 
        &
        \\
        Hierarchical \newline Recurrent (HRE) \newline \todo{reference}
        &$ \displaystyle
            \begin{aligned}
                u_t &= \text{LSTM}(U_t) \\
                h_t &= \text{LSTM}([u_i]_{i=1}^{t-1})
            \end{aligned}
        $ 
        &
        & 
        &
        \\
        Memory Network (MN) \newline \todo{reference}
        &$ \displaystyle
            \begin{aligned}
                u_t &= \text{LSTM}(U_t) \\
                h_t &= \text{LSTM}([u_i]_{i=1}^{t-1})
            \end{aligned}
        $ 
        &
        &
        &
        \\
        \midrule
        History-Agnostic (HAE-T) & & & & \\
        History-Aware (HE-T) & & & & \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    \vspace*{\captionReduceTop}
    \caption{
        Component Instantiations for \simmc Models.
    }
    \vspace*{\captionReduceBot}
    \label{tab:model_components}
\end{table}

==> tex_modules/tables/results_dst.tex <==
\begin{wraptable}{l}{0.32\textwidth}
    \vspace{-10pt}
    \scalebox{0.79}{
    \setlength\tabcolsep{3.5pt}
    \begin{tabular}{lcc}
    \toprule[\heavyrulewidth]
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{DST}} \\ 
    \cmidrule(r){2-3}
     & Intent.F1$\uparrow$  & Slot.F1$\uparrow$  \\
    \midrule
    \multicolumn{3}{c}{\furniture}  \\
    \midrule
    TRADE & - & 45.5 \\
    SimpleTOD & \textbf{75.0} & 50.1 \\
    SimpleTOD+MM & 74.1 & \textbf{60.2} \\
    \midrule
    \multicolumn{3}{c}{\fashion}  \\
    \midrule
    TRADE & - & 32.8 \\
    SimpleTOD & 56.5 & 37.3 \\
    SimpleTOD+MM & \textbf{59.1} & \textbf{43.5} \\
    \bottomrule[\heavyrulewidth]
    \end{tabular}
    }
    \captionof{table}{
        Results for: \textbf{Dialog State Tracking (DST)}, measured with intent and slot prediction F1.
    }
\label{tab:results_dst}
\end{wraptable}
\vspace{-10pt}


==> tex_modules/tables/results_simmc_elaborate.tex <==
\begin{table*}[t]
    \begin{center}
        \scalebox{0.80}{
        \begin{tabular}{
            p{0.30\textwidth}
            p{0.15\textwidth}
            p{0.15\textwidth}
            p{0.15\textwidth}
            p{0.15\textwidth}
            p{0.15\textwidth}
        }
        \toprule[\heavyrulewidth]
        \multirow{2}{*}{\textbf{Model}}
        & \multicolumn{3}{c}{\textbf{Action Prediction}}
        & \multicolumn{2}{c}{\textbf{Response Generation}} \\
        & Accuracy & Perplexity & Attr. Accuracy
        & BLEU & Perplexity \\
        \midrule
        \multicolumn{6}{c}{\furniture}\\
        \midrule
        TD-IDF & xxxx & xxxx & xxxx & xxxx & xxx\\
         \quad -AC, MC 
            & \reportval{9.73}{0.09}
            & \reportval{2.39}{0.09}
            & \reportval{73.8}{0.3}
            & xxxx
            & \reportval{60.2}{0.4}\\
        \cdashlinelr{1-6}
        HAE
            & \reportval{8.65}{0.07}
            & \reportval{2.86}{0.05}
            & \reportval{75.5}{0.6}
            & xxxx
            & \reportval{62.1}{0.9}\\
        \quad -AC, MC 
            & \reportval{8.67}{0.09}
            & \reportval{2.13}{0.11}
            & \reportval{74.4}{0.9}
            & xxxx
            & \reportval{55.5}{0.9}\\
        \cdashlinelr{1-6}
        HRE 
            & \reportval{9.14}{0.21}
            & \reportval{2.13}{0.13}
            & \reportval{76.8}{0.7}
            & xxxx
            & \reportval{61.9}{0.6}\\
        \quad -AC, MC 
            & \reportval{9.03}{0.02}
            & \reportval{2.03}{0.00}
            & \reportval{74.8}{0.2}
            & xxxx
            & \reportval{56.0}{0.5}\\
        \cdashlinelr{1-6}
        MN 
            & \reportval{8.74}{0.07}
            & \reportval{2.55}{0.31}
            & \reportval{76.1}{0.3}
            & xxxx
            & \reportval{61.6}{1.3}\\
        \quad -AC, MC 
            & \reportval{8.73}{0.09}
            & \reportval{2.08}{0.04}
            & \reportval{74.5}{0.6}
            & xxxx
            & \reportval{57.4}{1.2}\\
        \cdashlinelr{1-6}
        T-HAE 
            & \reportval{8.09}{0.01}
            & \reportval{2.06}{0.03}
            & \reportval{77.2}{0.3}
            & xxxx
            & \reportval{59.8}{0.5}\\
        \quad -AC, MC 
            & \reportval{8.08}{0.03}
            & \reportval{2.06}{0.02}
            & \reportval{75.0}{0.2}
            & xxxx
            & \reportval{55.1}{0.6}\\
        \midrule
        \multicolumn{6}{c}{\fashion}\\
        \midrule
        TD-IDF & xxxx & xxxx & xxxx & xxxx \\
        \quad -AC -MC & xxxx & xxxx & xxxx & xxxx \\
        \cdashlinelr{1-6}
        HAE & xxxx & xxxx & xxxx & xxxx \\
        \quad -AC -MC & xxxx & xxxx & xxxx & xxxx \\
        \cdashlinelr{1-5}
        HRE & xxxx & xxxx & xxxx & xxxx \\
        \quad -AC -MC & xxxx & xxxx & xxxx & xxxx \\
        \cdashlinelr{1-5}
        MN & xxxx & xxxx & xxxx & xxxx \\
        \quad -AC -MC & xxxx & xxxx & xxxx & xxxx \\
        \cdashlinelr{1-5}
        T-HAE & xxxx & xxxx & xxxx & xxxx \\
        \quad -AC -MC & xxxx & xxxx & xxxx & xxxx \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
    }
    \end{center}
    \vspace*{\captionReduceTop}
    \caption{Results on \furniture and \fashion. \todo{Fill the rest later.}}
    \label{tab:results_elaborate}
    \vspace*{\captionReduceBot}
\end{table*}

==> tex_modules/tables/task_definitions.tex <==
\begin{table*}[t]
    \begin{center}
        \scalebox{0.8}{
        \setlength\tabcolsep{5pt}
        \begin{tabular}{
            p{0.33\textwidth}p{0.48\textwidth}p{0.35\textwidth}
        }
        \toprule[\heavyrulewidth]
        \textbf{Task Name}  & \textbf{Description} &  \textbf{Evaluation} \\
        \midrule
        \textbf{Assistant Action Selection (Structural API Call Prediction)}
        &
        Given user utterances, predict the correct Assistant API action(s) (classification)
        &
        Perplexity, Mean Average Precision, (Human Evaluation)  \\
        \midrule
        \textbf{Response Generation}
        & Given user utterances and/or ground-truth 
        APIs, generate Assistant responses or retrieve from a candidate pool
        &
        Generation: BLEU, Perplexity, Human Evaluation (Naturalness, etc.); Retrieval: Accuracy@k, Entropy\\
        \midrule
        \textbf{Dialog State Tracking}
        &
        Given user utterances, track user belief states across multiple turns
        & 
        Intent F1, Slot F1 \\
        \bottomrule[\heavyrulewidth]
        \end{tabular}
        }
    \end{center}
    %\vspace*{\captionReduceTop}
    \caption{Overview of tasks enabled by our \simmc datasets.}
    \vspace*{\captionReduceBot}
    \label{tab:task_definitions}
\end{table*}
